Using non-Gaussian quantum states for detection of a given phase shift

Injecting a non-Gaussian (Fock or Shr\"odinger cat) quantum state into the dark port of a two-arm interferometer and a strong classical light into the bright one, it is possible, in principle, to detect a given phase shift unambiguously using the orthogonality between the original and displaced in the interferometer non-Gaussian states. The optical losses degrade the sensitivity, introducing the finite "false positive" and "false negative" detection errors. However, using the state-of-art photodetectors, it is still possible to obtain better detection fidelity than in the case of Gaussian quantum states.

==> mycolors.tex <==
\newcommand{\dr}{\color{Red4}}
\newcommand{\dg}{\color{Green4}}
\newcommand{\db}{\color{Blue3}}
\newcommand{\dm}{\color{Magenta4}}
\newcommand{\dc}{\color{Cyan4}}



==> mymac.tex <==
\emergencystretch=10pt

%\newcommand{\DIARY}{/home/science/diary}
%\newcommand{\PARATRNS}{/home/science/diary/paratrns}
%\newcommand{\SQUEEZE}{/home/science/diary/paratrns/squeeze}

%\setlength{\columnseprule}{0.4pt}
%\numberwithin{equation}{section}

\newcommand{\remark}[1]{\begin{flushright}{\large\it#1}\nopagebreak\end{flushright}}
%\newcommand{\dated}[1]{\ {\it(#1)}}
\newcommand{\dated}[1]{{\ (#1)}}
%\newcommand{\dated}[1]
%  {\begin{wrapfigure}{r}{2cm}{\small\it #1}\end{wrapfigure}}

\newcommand{\ie}{{\it i.e.\,}}
\newcommand{\eg}{{\it e.g.\,}}
\newcommand{\etc}{{\it etc}}

\newcommand{\HugeBiggl}[1]{\text{\Huge{$\Biggl#1$}}}
\newcommand{\hugeBiggl}[1]{\text{\huge{$\Biggl#1$}}}
\newcommand{\LARGEBiggl}[1]{\text{\LARGE{$\Biggl#1$}}}
\newcommand{\LargeBiggl}[1]{\text{\Large{$\Biggl#1$}}}
\newcommand{\largeBiggl}[1]{\text{\large{$\Biggl#1$}}}

\newcommand{\HugeBiggr}[1]{\text{\Huge{$\Biggr#1$}}}
\newcommand{\hugeBiggr}[1]{\text{\huge{$\Biggr#1$}}}
\newcommand{\LARGEBiggr}[1]{\text{\LARGE{$\Biggr#1$}}}
\newcommand{\LargeBiggr}[1]{\text{\Large{$\Biggr#1$}}}
\newcommand{\largeBiggr}[1]{\text{\large{$\Biggr#1$}}}

% \newcommand{\sh}{\sinh}
% \newcommand{\ch}{\cosh}
% \renewcommand{\th}{\tanh}
\newcommand{\nf}{\nicefrac}
\newcommand{\arccot}{\mathop{\rm arccot}\nolimits}
\newcommand{\const}{\mathop{\rm const}\nolimits}
\newcommand{\Sp}{\mathop{\rm Sp}\nolimits}
\newcommand{\Tr}{\mathop{\rm Tr}\nolimits}
\newcommand{\Det}{\mathop{\rm Det}\nolimits}
\newcommand{\Var}{\mathop{\rm Var}\nolimits}
\newcommand{\Cov}{\mathop{\rm Cov}\nolimits}
\newcommand{\sinc}{\mathop{\rm sinc}\nolimits}
\newcommand{\sign}{\mathop{\rm sign}\nolimits}
\newcommand{\hyphen}{\mathbin{\text{-}}}
\newcommand{\ntimes}{\!\times\!}
\newcommand{\symp}{\mathbin{\!\circ\!}}

\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\Re}{\mathop{\rm Re}\nolimits}
\renewcommand{\Im}{\mathop{\rm Im}\nolimits}
\renewcommand{\mod}{\mathbin{\rm mod}}

%\newcommand{\ve}[1]{\vec{\vphantom{N}#1}}
%\newcommand{\ve}[1]{\mathbf{#1}}

\newcommand{\hence}{\ \Rightarrow\ }
\newcommand{\from}{\ \Leftarrow\ }
\newcommand{\logequiv}{\ \Leftrightarrow\ }
\newcommand{\see}[2]{\stackrel{\text{#1}}{#2}}

\newcommand{\neswarrow}{{\nearrow\hspace{-1em}\swarrow}}
\newcommand{\nwsearrow}{{\nwarrow\hspace{-1em}\searrow}}

\newcommand{\dsum}{\displaystyle\sum}

\newcommand{\dint}{\displaystyle\int}
\newcommand{\intinfty}{\displaystyle\int_{-\infty}^{\infty}\!}
\newcommand{\intOinfty}{\displaystyle\int_{0}^{\infty}\!}
\newcommand{\fourie}[1]{\displaystyle\int_{-\infty}^{\infty}#1\,\dfrac{d\omega}{2\pi}}

\newcommand{\fulldiff}[2]{\dfrac{d#1}{d#2}}
\newcommand{\fulld}[2]{\dfrac{d#1}{d#2}}
\newcommand{\fulldd}[2]{\dfrac{d^2#1}{d#2^2}}
\newcommand{\partdiff}[2]{\dfrac{\partial#1}{\partial#2}}
\newcommand{\partd}[2]{\dfrac{\partial#1}{\partial#2}}
\newcommand{\partdd}[2]{\dfrac{\partial^2#1}{\partial#2^2}}

\newcommand{\contfrac}[2]{\rightsquigarrow\frac{#1}{#2}}

%\newcommand{\E}[1]{\times10^{#1}}

\newcommand{\hamilt}{\hat{\mathcal{H}}}
\newcommand{\evol}{\hat{\mathcal{U}}}

% \newcommand{\dag}{\dagger}
\newcommand{\dagsq}{{\dagger2}}
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\bracket}[2]{\langle{#1}|{#2}\rangle}
\newcommand{\mean}[1]{\langle{#1}\rangle}
\newcommand{\Bra}[1]{\left\langle{#1}\right|}
\newcommand{\Ket}[1]{\left|{#1}\right\rangle}
\newcommand{\bigbracket}[2]{\bigl\langle#1\bigm|#2\bigr\rangle}
\newcommand{\Bigbracket}[2]{\Bigl\langle#1\Bigm|#2\Bigr\rangle}
\newcommand{\biggbracket}[2]{\biggl\langle#1\biggm|#2\biggr\rangle}
\newcommand{\Biggbracket}[2]{\Biggl\langle#1\Biggm|#2\Biggr\rangle}
\newcommand{\Mean}[1]{\left\langle#1\right\rangle}

\newcommand{\spinor}[2]{\begin{pmatrix}#1 \\ #2\end{pmatrix}}
\newcommand{\cspinor}[2]{\begin{pmatrix}#1 & #2\end{pmatrix}}
\newcommand{\svector}[2]{\begin{pmatrix}#1 \\ #2 \end{pmatrix}}
\newcommand{\rvector}[2]{\begin{pmatrix}#1 & #2 \end{pmatrix}}
\newcommand{\smatrix}[4]{\begin{pmatrix}#1 & #2 \\ #3 & #4\end{pmatrix}}
\newcommand{\srvector}[2]{\begin{pmatrix*}[r]#1 \\ #2\end{pmatrix*}}
\newcommand{\srmatrix}[4]{\begin{pmatrix*}[r]#1 & #2 \\ #3 & #4\end{pmatrix*}}
\newcommand{\threevector}[3]{\begin{pmatrix}#1 \\ #2 \\ #3\end{pmatrix}}
\newcommand{\fvector}[4]{\begin{pmatrix}#1 \\ #2 \\ #3 \\ #4\end{pmatrix}}
\newcommand{\fourvector}[4]{\begin{pmatrix}#1 \\ #2 \\ #3 \\ #4\end{pmatrix}}
\newcommand{\blockvector}[2]{\left(\begin{array}{c}
  #1 \\[0.5ex] \hline \\[-2.5ex] #2
\end{array}\right)}
\newcommand{\blockrvector}[2]{\left(\begin{array}{c|c}
  #1 & #2
\end{array}\right)}
\newcommand{\blockmatrix}[4]{\left(\begin{array}{c|c}
  #1 & #2 \\[0.5ex] \hline \\[-2.5ex] #3 & #4
\end{array}\right)}

\newcommand{\horzarrow}{\leftrightarrow}
\newcommand{\vertarrow}{\updownarrow}
\newcommand{\leftcirc}{\circlearrowleft}
\newcommand{\rightcirc}{\circlearrowright}
\newcommand{\svup}{\genfrac{(}{)}{0pt}{}{1}{0}}
\newcommand{\svdown}{\genfrac{(}{)}{0pt}{}{0}{1}}
\newcommand{\kethorz}{\ket{\!\leftrightarrow}}
\newcommand{\ketvert}{\ket{\!\updownarrow}}
\newcommand{\ketcircleft}{\ket{!\circlearrowleft}}
\newcommand{\ketcircright}{\ket{!\circlearrowright}}
\newcommand{\brahorz}{\bra{\leftrightarrow\!}}
\newcommand{\bravert}{\bra{\updownarrow\!}}
\newcommand{\bracircleft}{\bra{!\circlearrowleft}}
\newcommand{\bracircright}{\bra{!\circlearrowright}}
\newcommand{\ketup}{\ket{\!\uparrow}}
\newcommand{\braup}{\bra{\uparrow\!}}
\newcommand{\ketdn}{\ket{\!\downarrow}}
\newcommand{\bradn}{\bra{\downarrow\!}}
\newcommand{\ketlf}{\ket{\!\leftarrow}}
\newcommand{\bralf}{\bra{\leftarrow\!}}
\newcommand{\ketrt}{\ket{\!\rightarrow}}
\newcommand{\brart}{\bra{\rightarrow\!}}
\newcommand{\quot}[1]{``#1\text{''}}
\newcommand{\defis}{\,\text{-}\,}

\newcommand{\snr}{{\dfrac{s}{n}}}

\newcommand{\textat}[3]{\put({#1},{#2}){\makebox(0,0)[c,c]{#3}}}

\newcommand{\kT}{\kappa_B T}
\newcommand{\cc}{\mathrm{c.c.}}
\newcommand{\hc}{\mathrm{h.c.}}
\newcommand{\CC}{\mathrm{C.C.}}

